C$^2$U in RAG: Compositional Concept Unlearning in Retrieval-Augmented Generation

Retrieval-augmented generation can expose unwanted concepts through retrieved evidence even when the generator is moderated. We study query-side concept suppression with a fixed encoder and document index. Compositional Concept Unlearning (C$^2$U) routes a profile-derived direction through an augmented atom bank, adding only a bounded edited-minus-original delta to the raw query. Across five datasets, four encoders, and three seeds, the validation-selected configuration reduces pooled binary target Hit@5 by 4.25 percentage points with non-positive control degradation and target-exposure changes. Under the evaluated query transforms, it suppresses target density without increasing budgeted control-query exposure. Separately, ArXiv four-concept composition improves over an averaged-direction comparator after independent validation gates and first-use test evaluation.

==> tables/case_excerpt_arr_v1.tex <==
\begin{table}[t]
\centering
\small
\definecolor{arrHero}{HTML}{E9C46B}
\definecolor{caseGray}{gray}{0.42}
\caption{\textbf{One retrieval example where a target label exits the top-5 (ArXiv).} Selected by the pre-registered rule (base hit $\to$ method miss, maximum target-cosine drop, deterministic tie-breaks), frozen before any query text was read; a selected successful case, not a typical sample. Full five-dataset table: Table~\ref{tab:case_study}.}
\label{tab:case_excerpt}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lp{5.2cm}@{}}
\toprule
\textbf{Query} & Research about AI-based code generators have gained a fundamental role in assisting developers\dots{} \\
\textbf{Target concept} & \colorbox{arrHero!25}{System Attacks} \\
\textbf{Base top-5} & \textcolor{caseGray}{Software Engineering}, \textcolor{caseGray}{Software Engineering}, \textcolor{caseGray}{Software Engineering}, \colorbox{arrHero!25}{System Attacks}, \textcolor{caseGray}{Artificial Intelligence} \\
\textbf{Edited top-5} & \textcolor{caseGray}{Software Engineering}, \textcolor{caseGray}{Software Engineering}, \textcolor{caseGray}{Artificial Intelligence}, \textcolor{caseGray}{Software Engineering}, \textcolor{caseGray}{Machine Translation} \\
\textbf{Edit angle} & 0.200 rad \\
\bottomrule
\end{tabular}
\end{table}

